DiffCAD: Weakly-Supervised Probabilistic CAD Model Retrieval and Alignment from an RGB Image

Perceiving 3D structures from RGB images based on CAD model primitives can enable an effective, efficient 3D object-based representation of scenes. However, current approaches rely on supervision from expensive annotations of CAD models associated with real images, and encounter challenges due to the inherent ambiguities in the task -- both in depth-scale ambiguity in monocular perception, as well as inexact matches of CAD database models to real observations. We thus propose DiffCAD, the first weakly-supervised probabilistic approach to CAD retrieval and alignment from an RGB image. We formulate this as a conditional generative task, leveraging diffusion to learn implicit probabilistic models capturing the shape, pose, and scale of CAD objects in an image. This enables multi-hypothesis generation of different plausible CAD reconstructions, requiring only a few hypotheses to characterize ambiguities in depth/scale and inexact shape matches. Our approach is trained only on synthetic data, leveraging monocular depth and mask estimates to enable robust zero-shot adaptation to various real target domains. Despite being trained solely on synthetic data, our multi-hypothesis approach can even surpass the supervised state-of-the-art on the Scan2CAD dataset by 5.9% with 8 hypotheses.

==> figs/figure_teaser.tex <==
% Teaser
\begin{figure}
\twocolumn[{%
\renewcommand\twocolumn[1][]{#1}%
\maketitle
\begin{center}
    \centering
    \includegraphics[width=0.98\textwidth]{figs/teaser_compressed.pdf}
    \caption{
    We introduce \OURS, a weakly-supervised probabilistic approach for CAD model retrieval and alignment to a single RGB image.
    Unlike existing methods that require expensive CAD associations to real images for supervision, our approach is only trained on synthetic data, yet it can demonstrate superior performance on real-world datasets. 
    }
    \label{figure:teaser}
\end{center}%
}]
\end{figure}

==> tables/confidence_retrieval.tex <==
\begin{table}[ht]
    \caption{
        \textbf{Confidence Filtering of Probabilistic Retrieval}. Given initial retrieval candidates, we calculate the variance and filter out the high-variance predictions by setting the 2-$\sigma$ threshold. Our probabilistic pipeline shows improved results when only considering high-confidence candidates.
        }
        \label{table:retrieval_confidence}
    \centering
    \resizebox{0.47\textwidth}{!}
        {
        \begin{tabular}{l c *{6}{>{\centering\arraybackslash}m{0.08\linewidth}} c}
            \hline 
            Method                                 &\#hypotheses              &        bed       &      bkshlf      &      cabinet     &     chair        &      sofa        &       table      & avg$\uparrow$ \\
            \hline 
            \Ours w/o filtering      & 8                        &        0.075      &      0.064       &      0.079       &      0.075       &      0.066       &       0.089      &   0.075      \\
            \textbf{Ours w/ filtering}                          & 8         &   \textbf{0.072}  &   \textbf{0.066}  &   \textbf{0.055}  &   {0.068}  &    \textbf{0.058} &  \textbf{0.073}  &\textbf{0.065} \\
            \hline
            
        \end{tabular}
        }
\end{table}


